Towards The Implicit Bias on Multiclass Separable Data Under Norm Constraints

Implicit bias induced by gradient-based algorithms is essential to the generalization of overparameterized models, yet its mechanisms can be subtle. This work leverages the Normalized Steepest Descent} (NSD) framework to investigate how optimization geometry shapes solutions on multiclass separable data. We introduce NucGD, a geometry-aware optimizer designed to enforce low rank structures through nuclear norm constraints. Beyond the algorithm itself, we connect NucGD with emerging low-rank projection methods, providing a unified perspective. To enable scalable training, we derive an efficient SVD-free update rule via asynchronous power iteration. Furthermore, we empirically dissect the impact of stochastic optimization dynamics, characterizing how varying levels of gradient noise induced by mini-batch sampling and momentum modulate the convergence toward the expected maximum margin solutions.Our code is accessible at: https://github.com/Tsokarsic/observing-the-implicit-bias-on-multiclass-seperable-data.

==> abstract.tex <==
\begin{abstract}

\end{abstract}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk --shell-escape -pdf \"$_[0]\"" );
    }
}

==> math_commands.tex <==
\usepackage{amsmath,bm,dsfont,amssymb,xspace}

\newtheorem{thm}{Theorem}
\newtheorem{remark}{Remark}
\newtheorem{assumption}{Assumption}
%\newtheorem{lemma}[thm]{Lemma}
\newtheorem{cor}[thm]{Corollary}
%\newtheorem{proposition}[thm]{Proposition}
\newtheorem{example}{Example}
%\newtheorem{definition}{Definition}
%\newtheorem{theorem}{Theorem}
%\newtheorem{algorithm}{Algorithm}
\usepackage{apptools}
\usepackage{booktabs}
\usepackage{threeparttable}
\AtAppendix{\counterwithin{thm}{section}}
\newcommand{\q}{\frac{N-S}{S(N-1)}}


\newcommand{\one}{\mathds{1}_n}
\newcommand{\R}{n^{-1}\mathds{1}_n \mathds{1}_n^T}

\newcommand{\va}{{\mathbf{a}}}
\newcommand{\vb}{{\mathbf{b}}}
\newcommand{\vc}{{\mathbf{c}}}
\newcommand{\vd}{{\mathbf{d}}}
\newcommand{\ve}{{\mathbf{e}}}
\newcommand{\vf}{{\mathbf{f}}}
\newcommand{\vg}{{\mathbf{g}}}
\newcommand{\vh}{{\mathbf{h}}}
\newcommand{\vi}{{\mathbf{i}}}
\newcommand{\vj}{{\mathbf{j}}}
\newcommand{\vk}{{\mathbf{k}}}
\newcommand{\vl}{{\mathbf{l}}}
\newcommand{\vm}{{\mathbf{m}}}
\newcommand{\vn}{{\mathbf{n}}}
\newcommand{\vo}{{\mathbf{o}}}
\newcommand{\vp}{{\mathbf{p}}}
\newcommand{\vq}{{\mathbf{q}}}
\newcommand{\vr}{{\mathbf{r}}}
\newcommand{\vs}{{\mathbf{s}}}
\newcommand{\vt}{{\mathbf{t}}}
\newcommand{\vu}{{\mathbf{u}}}
\newcommand{\vv}{{\mathbf{v}}}
\newcommand{\vw}{{\mathbf{w}}}
\newcommand{\vx}{{\mathbf{x}}}
\newcommand{\vy}{{\mathbf{y}}}
\newcommand{\vz}{{\mathbf{z}}}

\newcommand{\vA}{{\mathbf{A}}}
\newcommand{\vB}{{\mathbf{B}}}
\newcommand{\vC}{{\mathbf{C}}}
\newcommand{\vD}{{\mathbf{D}}}
\newcommand{\vE}{{\mathbf{E}}}
\newcommand{\vF}{{\mathbf{F}}}
\newcommand{\vG}{{\mathbf{G}}}
\newcommand{\vH}{{\mathbf{H}}}
\newcommand{\vI}{{\mathbf{I}}}
\newcommand{\vJ}{{\mathbf{J}}}
\newcommand{\vK}{{\mathbf{K}}}
\newcommand{\vL}{{\mathbf{L}}}
\newcommand{\vM}{{\mathbf{M}}}
\newcommand{\vN}{{\mathbf{N}}}
\newcommand{\vO}{{\mathbf{O}}}
\newcommand{\vP}{{\mathbf{P}}}
\newcommand{\vQ}{{\mathbf{Q}}}
\newcommand{\vR}{{\mathbf{R}}}
\newcommand{\vS}{{\mathbf{S}}}
\newcommand{\vT}{{\mathbf{T}}}
\newcommand{\vU}{{\mathbf{U}}}
\newcommand{\vV}{{\mathbf{V}}}
\newcommand{\vW}{{\mathbf{W}}}
\newcommand{\vX}{{\mathbf{X}}}
\newcommand{\vY}{{\mathbf{Y}}}
\newcommand{\vZ}{{\mathbf{Z}}}

\newcommand{\cA}{{\mathcal{A}}}
\newcommand{\cB}{{\mathcal{B}}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\cD}{{\mathcal{D}}}
\newcommand{\cE}{{\mathcal{E}}}
\newcommand{\cF}{{\mathcal{F}}}
\newcommand{\cG}{{\mathcal{G}}}
\newcommand{\cH}{{\mathcal{H}}}
\newcommand{\cI}{{\mathcal{I}}}
\newcommand{\cJ}{{\mathcal{J}}}
\newcommand{\cK}{{\mathcal{K}}}
\newcommand{\cL}{{\mathcal{L}}}
\newcommand{\cM}{{\mathcal{M}}}
\newcommand{\cN}{{\mathcal{N}}}
\newcommand{\cO}{{\mathcal{O}}}
\newcommand{\cP}{{\mathcal{P}}}
\newcommand{\cQ}{{\mathcal{Q}}}
\newcommand{\cR}{{\mathcal{R}}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\cU}{{\mathcal{U}}}
\newcommand{\cV}{{\mathcal{V}}}
\newcommand{\cW}{{\mathcal{W}}}
\newcommand{\cX}{{\mathcal{X}}}
\newcommand{\cY}{{\mathcal{Y}}}
\newcommand{\cZ}{{\mathcal{Z}}}

\newcommand{\EE}{\mathbb{E}}
\newcommand{\RR}{\mathbb{R}}

\newcommand{\pushsum}{{\sc Push-Sum}\xspace}
\newcommand{\pushonly}{{\sc Push-Only}\xspace}
\newcommand{\pushpull}{{\sc Push-Pull}\xspace}
\newcommand{\pushdg}{{\sc Push-DIGing}\xspace}
\newcommand{\pullonly}{{\sc Pull-Only}\xspace}
\newcommand{\AB}{{\sc AB}\xspace}
\newcommand{\extrapush}{{\sc EXTRA-Push}\xspace}
\newcommand{\dextra}{{\sc DEXTRA}\xspace}
\newcommand{\addopt}{{\sc ADD-OPT}\xspace}
\newcommand{\saddopt}{{\sc S-ADDOPT}\xspace}
\newcommand{\ab}{{\sc AB}\xspace}
\newcommand{\subpush}{{\sc Subgradient-Push}\xspace}
\newcommand{\sgdpush}{{\sc SGD-Push}\xspace}

\newcommand{\norm}[1]{\| #1 \|}
\newcommand{\ip}[1]{\left\langle#1\right\rangle}
\newcommand{\eg}{{\em e.g.\xspace}}
\newcommand{\ie}{{\em i.e.\xspace}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\lly}[1]{{\color{blue}[lly: #1]}}
\newcommand{\ky}[1]{\textcolor{red}{[KY: #1]}}
\newcommand{\xh}[1]{\textcolor{brown}{[XH: #1]}}
\definecolor{gan}{RGB}{128,128,255}
\newcommand{\gan}[1]{\textcolor{gan}{[#1]}}


\newcommand{\Rowonly}{{\sc Row-Only}\xspace}
\newcommand{\Colonly}{{\sc Col-Only}\xspace}
\newcommand{\pullsum}{{\sc Pull-Sum}\xspace}
\newcommand{\pulldiag}{{\sc Pull-Diag}\xspace}
\newcommand{\frsd}{{\sc FRSD}\xspace}
\newcommand{\frozen}{{\sc FROZEN}\xspace}
\newcommand{\pulldg}{{\sc Pull-DIGing}\xspace}

==> temp.tex <==
% \begin{lemma}[\sc \small Consensus of x]\label{lem:coarse-x}
% Suppose Assumption~\ref{ass:smooth},~\ref{ass:gradient oracle} and Proposition~\ref{prop:perron} hold. For any $T\ge 0$, we have
%     \begin{align*}
%         \sum_{k=0}^T\EE[\norm{\Delta_x^{(k+1)}}^2]&\le 2\alpha^2s_A^2\sum_{k=0}^T\EE[\norm{\Delta_y^{(k)}}^2]\\
%         &\quad+2\alpha^2n^2s_A^2\sum_{k=0}^T\EE[\norm{\overline{\nabla f}^{(k)}}^2]+2n\alpha^2s_A^2(T+1)\sigma^2
%     \end{align*}
% \end{lemma}
% \begin{proof}
% First note that
% \begin{align*}
%     \Delta_x^{(k+1)} &= (I-A_\infty)\vx^{(k+1)}= (A-A_\infty)\vx^{(k)}-(I-A_\infty)\vy^{(k)}\\
%     &= \ldots = \sum_{i=0}^k (A^{k-i}-A_\infty)\vy^{(i)}\\
%     &=\sum_{i=0}^k (A^{k-i}-A_\infty)\Delta_y^{(i)}+\sum_{i=0}^k (A^{k-i}-A_\infty)n\pi_B \bar{g}^{(i)}
% \end{align*}

% Using the rolling sum lemma, we have
% \begin{align*}
%     \sum_{k=0}^T \norm{\Delta_x^{(k+1)}}_F^2 \le 2s_A^2 \sum_{k=0}^T\norm{\Delta_y^{(k+1)}}_F^2 +2n^2s_A^2\norm{\pi_B}^2\sum_{k=0}^T\norm{\bar{g}^{(k)}}_F^2.
% \end{align*}

% Note that $\EE[\norm{\bar{g}^{(k)}}_F^2]\le n^{-1}\sigma^2+\EE[\norm{\overline{\nabla f}^{(k)}}_F^2]$ and $\norm{\pi_B}\le 1$, we finish the proof.
% \end{proof}



% \begin{lemma}[\sc \small Consensus of y]\label{lem:coarse-y}
% Suppose Assumption~\ref{ass:smooth},~\ref{ass:gradient oracle} and Proposition~\ref{prop:perron} hold. For any $T\ge 0$, when $\alpha \le \frac{1}{6\sqrt{n}s_As_BL}$, we have

%         \begin{align*}
%     \sum_{k=0}^T \norm{\Delta_y^{(k+1)}}_F^2\le 30ns_B^2(T+1)\sigma^2+8ns_B^2L\Delta+108\alpha^2L^2 n^3s_A^2s_B^2\sum_{k=0}^T\EE[\norm{\overline{\nabla f}^{(k)}}_F^2]
% \end{align*}

% \end{lemma}

% \begin{proof}
%     \begin{align*}
%         \Delta_y^{(k+1)} &= (B-B_\infty)\Delta_y^{(k)}+(I-B_\infty)(\vg^{(k+1)}-\vg^{(k)})\\
%         &=\ldots = (B^{k+1}-B_\infty)\vg^{(0)}+\sum_{i=0}^k (B^{k-i}-B_\infty)(\vg^{(i+1)}-\vg^{(i)})
%     \end{align*}
% Using the rolling sum lemma, we have
% \begin{align*}
%     \sum_{k=0}^T \norm{\Delta_y^{(k+1)}}_F^2\le s_B^2\norm{\vg^{(0)}}+s_B^2 \sum_{k=0}^T\norm{\vg^{(k+1)}-\vg^{(k)}}_F^2 
% \end{align*}
% By Cauchy-Schwarz Inequality and our assumption for bounded noise, we have
% \begin{align*}
%     \EE[\norm{\vg^{(k+1)}-\vg^{(k)}}_F^2]&\le 6n\sigma^2+3\EE[\norm{\nabla f(\vx^{(k+1)})-\nabla f(\vx^{(k)})}_F^2]\\
%     &\le 6n\sigma^2+ 3L^2\EE[\norm{\vx^{(k+1)}-\vx^{(k)}}_F^2]
% \end{align*}
% Besides, $\EE[\norm{\vg^{(0)}}_F^2]\le 
% n\sigma^2 + \norm{\nabla f(\vx^{(0)})}_F^2\le n\sigma^2+2nL\Delta$. Therefore, we have 
% \begin{align}\label{eq:coarse y-1}
%     \sum_{k=0}^T \norm{\Delta_y^{(k+1)}}_F^2\le ns_B^2(6T+7)\sigma^2+2ns_B^2L\Delta+3s_B^2L^2\sum_{k=0}^T\EE[\norm{\vx^{(k+1)}-\vx^{(k)}}_F^2].
% \end{align}
% Since
% \begin{align}\label{eq:coarse y-2}
%     &\quad\EE[\norm{\vx^{(k+1)}-\vx^{(k)}}_F^2] = \EE[\norm{(A-I)\vx^{(k)}-\alpha \vy^{(k)}}_F^2]\\
%     &=\EE[\norm{(A-I)\Delta_x^{(k)}-\alpha \Delta_y^{(k)}+n\alpha \pi_B \bar{g}^{(k)} }_F^2]\nonumber\\
%     &\le 3\norm{A-I}_2^2\EE[\norm{\Delta_x^{(k)}}_F^2]+3\alpha^2 \EE[\norm{\Delta_y^{(k)}}_F^2]+3n\alpha^2\sigma^2+ 3n^2\alpha^2\EE[\norm{\overline{\nabla f}^{(k)}}_F^2],\nonumber
% \end{align}
% and $\norm{A-I}_2^2\le 2n$, we can apply~\eqref{eq:coarse y-2} to substitute the last term in~\eqref{eq:coarse y-1}. This produces
% \begin{align*}
%     &(1-9\alpha^2L^2s_B^2)\sum_{k=0}^T \norm{\Delta_y^{(k+1)}}_F^2\le ns_B^2(6T+7+9\alpha^2L^2 T)\sigma^2\\
%     &\quad+9ns_B^2L^2\sum_{k=0}^T\EE[\norm{\Delta_x^{(k)}}_F^2]+9\alpha^2L^2n^2s_B^2\sum_{k=0}^T\EE[\norm{\overline{\nabla f}^{(k)}}_F^2]+2ns_B^2L\Delta
% \end{align*}

% Using the conclusion of Lemma~\ref{lem:coarse-x}, this can be further transformed to
% \begin{align*}
%     &\quad(1-9\alpha^2L^2s_B^2-18\alpha^2L^2 ns_A^2s_B^2)\sum_{k=0}^T \norm{\Delta_y^{(k+1)}}_F^2\\
%     &\le ns_B^2(6T+7+9\alpha^2L^2 T+18\alpha^2L^2 ns_A^2T)\sigma^2+2ns_B^2L\Delta\\
%     &\quad+(9\alpha^2L^2n^2s_B^2+18\alpha^2L^2 n^3s_A^2s_B^2)\sum_{k=0}^T\EE[\norm{\overline{\nabla f}^{(k)}}_F^2]
% \end{align*}
% When $\alpha\le \frac{1}{6\sqrt{n}s_As_BL}$, this can be simplified to 
% \begin{align*}
%     \sum_{k=0}^T \norm{\Delta_y^{(k+1)}}_F^2\le 30ns_B^2(T+1)\sigma^2+8ns_B^2L\Delta+108\alpha^2L^2 n^3s_A^2s_B^2\sum_{k=0}^T\EE[\norm{\overline{\nabla f}^{(k)}}_F^2].
% \end{align*}
% \end{proof}
% \begin{lemma}[\sc\small More Precise Estimate]
    
% \end{lemma}
\section{Convergence Analysis of Power Iteration Direction}\label{proof}

Consider the algorithm proposed in \ref{alg:nucgd-real}, where we take a single step power iteration in one gradient step, $p_t = \frac{\bm{M}_t \bm{M}_t^T p_{t-1}}{\|\bm{M}_t \bm{M}_t^T p_{t-1}\|}$. Intuitively, the gap between the \emph{exact} principal left singular vector $u_t$ and \emph{empirical} principal left singular vector $p_t$ will fade when the algorithm converge. Here we establish a rough theoretical guarantee for the idea. 

We use the tangent of the angle (denoted by $\angle(\cdot, \cdot)$) to measure the similarity of two unit vectors, which can be transformed to cosine similarity easily. Assumptions are as below:
\begin{enumerate}
    \item[(i)] $\lim_{t\to\infty}\tan \angle(u_{t-1}, u_t)=0$; 
    \item[(ii)] $\frac{\sigma_2(\bm{M}_t)}{\sigma_1(\bm{M}_t)} \le \rho < 1$ uniformly hold for all $t$, where $\sigma_1(\bm{M}_t), \sigma_2(\bm{M}_t)$ are the first and second singular value of $\bm{M}_t$, $\rho$ is a constant;
    \item[(iii)] $\liminf_{t\to \infty}\tan \mid\angle(p_{t}, u_t)\mid = 0.$
    
\end{enumerate}
First we proof a lemma, stating the contraction property of power iteration:
\begin{lemma}
 $\mid\tan \angle(p_t, u_t)\mid \leq \rho^2 \mid\tan \angle(p_{t-1}, u_t)\mid, \quad \forall t \geq 1.$
\end{lemma}
\begin{proof}
Let $\sigma_1 \ge \sigma_2 \ge \dots \ge \sigma_{\min_(k, d)} \ge 0$ be the singular values of $\bm{M}_t$. Then the eigenvalues of $\bm{N}_t = \bm{M}_t \bm{M}_t^T$ are $\lambda_i = \sigma_i^2$ or zero. We decompose the vector $p_{t-1}$ in the basis of the eigenvectors $\{u_i\}_{i=1}^k$ of $\bm{N}_t$:
\[
p_{t-1} = c_1 u_t + \sum_{i=2}^k c_i u_i,
\]
where $v_i$ are eigenvectors corresponding to $\lambda_i$ for $i \ge 2$. When $c_1=0$, the inequality trivially hold. For $c_1 \neq 0$, we have:
\[
\mid\tan \angle(p_{t-1}, u_t)\mid = \frac{\sqrt{\sum_{i=2}^k c_i^2}}{|c_1|}.
\]
After applying $\bm{N}_t$, the unnormalized vector is $\tilde{p}_t = c_1 \lambda_1 u_t + \sum_{i=2}^k c_i \lambda_i v_i$. The tangent of the new angle is:
\[
\mid\tan \angle(p_t, u_t)\mid = \frac{\sqrt{\sum_{i=2}^k c_i^2 \lambda_i^2}}{|c_1| \lambda_1}.
\]
Applying $\sqrt{\sum_{i=2}^k c_i^2 \lambda_i^2} \le \lambda_2 \sqrt{\sum_{i=2}^k c_i^2}$, we obtain:
\[
\mid\tan \angle(p_t, u_t)\mid \le \frac{\lambda_2}{\lambda_1} \frac{\sqrt{\sum_{i=2}^k c_i^2}}{|c_1|} = \frac{\sigma_2^2}{\sigma_1^2} \tan \mid\angle(p_{t-1}, u_t)\mid \le \rho^2 \tan \mid\angle(p_{t-1}, u_t)\mid.
\]
\end{proof}
\begin{theorem}
        Under the assumptions (i)$\sim$(iii), we have $\lim_{t \to \infty} \langle p_t, u_t \rangle = 1.$
\end{theorem}
\begin{proof}
Denote $\delta = \mid \tan\angle(u_t, u_{t-1})\mid$, $e_t = \mid\tan\angle(p_t, u_t)\mid$. Then $\liminf_{t\to\infty}\delta_t e_t=0$, so $e_{t-1}\delta_t\leq 1-\rho$ holds for infinite times.
First, consider the angle between the previous estimate $p_{t-1}$ and the current true eigenvector $u_t$. By the triangle inequality for angles in a metric space:
\[
\angle(p_{t-1}, u_t) \le \angle(p_{t-1}, u_{t-1}) + \angle(u_{t-1}, u_t).
\]
The angles are all acute by Assumption (iii), we can apply the tangent function:
\begin{equation} \label{eq:angle_drift}
    \tan \angle(p_{t-1}, u_t) \le \frac{\tan \angle(p_{t-1}, u_{t-1}) + \tan \angle(u_{t-1}, u_t)}{1 - \tan \angle(p_{t-1}, u_{t-1}) \tan \angle(u_{t-1}, u_t)} \leq \frac{\tan \angle(p_{t-1}, u_{t-1}) + \tan \angle(u_{t-1}, u_t)}{1 -\delta_t}.
\end{equation}

Next, we consider the contraction property of the Power Iteration step. Since $p_t$ is obtained by applying $M_t M_t^T$ to $p_{t-1}$, the tangent of the error angle contracts by the ratio of the eigenvalues (which are the squares of the singular values):
\begin{equation} \label{eq:contraction}
    \tan \angle(p_t, u_t) \le \left( \frac{\sigma_2(M_t)}{\sigma_1(M_t)} \right)^2 \tan \angle(p_{t-1}, u_t) \le \rho^2 \tan \angle(p_{t-1}, u_t).
\end{equation}

Let $e_t = \tan \angle(p_t, u_t)$. Combining \eqref{eq:angle_drift} and \eqref{eq:contraction}, and substituting $\delta_t = \tan \angle(u_{t-1}, u_t)$, we obtain the recursive inequality:
\[
e_t \le \rho^2 \cdot \frac{e_{t-1} + \delta_t}{1 -  \delta_t}\leq \frac{\rho^2}{1-c}(e_{t-1}+\delta_t)
\]
Since $\delta_t \to 0$ and $\frac{\rho^2}{1-c} < 1$, the sequence $e_t$ converges to 0 by Gronwall's inequality. Thus, $\angle(p_t, u_t) \to 0$, which implies $\langle p_t, u_t \rangle \to 1$.
\qed



\end{proof}

==> temp_proof.tex <==


\noindent \textbf{Assumptions:}
\begin{enumerate}
    \item[(A1)] \textbf{Smoothness of Objective:} The function $f$ is $L$-smooth, meaning its gradient is Lipschitz continuous: $\|\nabla f(X) - \nabla f(Y)\|_F \le L \|X - Y\|_F$.
    \item[(A2)] \textbf{Bounded Gradients:} The gradients are bounded during the trajectory, i.e., $\|\nabla f(W_t)\|_F \le G_{\max}$.
    \item[(A3)] \textbf{Uniform Spectral Gap:} The momentum matrix $M_t$ maintains a spectral gap: $\sigma_2(M_t) / \sigma_1(M_t) \le \rho < 1$.
    \item[(A4)] \textbf{Diminishing Step Size:} The step size sequence satisfies $\gamma_t \to 0$ (or we analyze the convergence at a stationary point where $\|W_{t+1} - W_t\| \to 0$).
\end{enumerate}

\noindent \textbf{Lemma 1 (Bound on Eigenvector Drift):}
Under Assumption (A1) and the NucGD update rules, the drift of the principal eigenvector of $A_t = M_t M_t^T$ satisfies:
\[
\delta_t := \tan \angle(u_{t-1}, u_t) \le C \cdot \|W_t - W_{t-1}\|_F
\]
where $C$ is a constant depending on $L$, $\mu$, and the spectral gap.

\noindent \textit{Proof of Lemma 1:}
\begin{enumerate}
    \item \textbf{Gradient Continuity:} By (A1), the change in gradient is bounded by the weight update:
    \[ \|\nabla f(W_t) - \nabla f(W_{t-1})\|_F \le L \|W_t - W_{t-1}\|_F. \]
    
    \item \textbf{Momentum Stability:} The momentum update is $M_t = \mu M_{t-1} + (1-\mu)\nabla f(W_t)$. The difference is:
    \[ M_t - M_{t-1} = \mu(M_{t-1} - M_{t-2}) + (1-\mu)(\nabla f(W_t) - \nabla f(W_{t-1})). \]
    Unrolling this recursion (and assuming initialization at 0), the change in $M_t$ is a weighted sum of past gradient changes. Since $\mu < 1$, this sum is dominated by the recent terms:
    \[ \|M_t - M_{t-1}\|_F \le \frac{1-\mu}{1-\mu} \sup_k \|\nabla f(W_k) - \nabla f(W_{k-1})\| \propto L \|W_t - W_{t-1}\|_F. \]
    
    \item \textbf{Matrix Perturbation:} Let $A_t = M_t M_t^T$. The perturbation $\|A_t - A_{t-1}\|_F$ is roughly bounded by $2\|M_t\| \|M_t - M_{t-1}\|$.
    
    \item \textbf{Davis-Kahan Theorem:} The rotation of the eigenvector is bounded by the matrix perturbation divided by the spectral gap ($g$):
    \[ \sin \angle(u_{t-1}, u_t) \le \frac{2\|A_t - A_{t-1}\|_F}{g} \le \frac{K \cdot L}{g} \|W_t - W_{t-1}\|_F. \]
    Thus, $\delta_t = O(\|W_t - W_{t-1}\|_F) = O(\gamma_t)$.
\end{enumerate}
\qed

\noindent \textbf{Theorem (Asymptotic Consistency):}
If the step size $\gamma_t$ is chosen such that $\delta_t \le \frac{1-\rho^2}{2}$ (which is satisfied for large $t$ as $\gamma_t \to 0$), then:
\[ \lim_{t \to \infty} \langle p_t, u_t \rangle = 1. \]

\noindent \textbf{Proof of Theorem:}
Let $e_t = \tan \angle(p_t, u_t)$.
From the geometry of subspace tracking and Power Iteration contraction:
\[
e_t \le \rho^2 \frac{e_{t-1} + \delta_t}{1 - e_{t-1} \delta_t}.
\]
Using \textbf{Lemma 1}, we substitute $\delta_t \le C \gamma_t$.
Since $\gamma_t \to 0$, there exists $T$ such that for all $t > T$, $\delta_t$ is small enough to ensure the denominator $1 - e_{t-1}\delta_t > \frac{1}{2}$.
The recurrence becomes:
\[
e_t \le (\rho^2 + \epsilon) e_{t-1} + C' \gamma_t.
\]
By the property of contracting sequences with vanishing perturbations (Toeplitz lemma logic), since $\gamma_t \to 0$, we conclude $e_t \to 0$.
\qed
